Stability of Planar Switched Systems under Delayed Event Detection

In this paper, we analyse the impact of delayed event detection on the stability of a 2-mode planar hybrid automata. We consider hybrid automata with a unique equilibrium point for all the modes, and we find the maximum delay that preserves stability of that equilibrium point. We also show for the class of hybrid automata treated that the instability of the equilibrium point for the equivalent hybrid automaton with delay in the transitions is equivalent to the existence of a closed orbit in the hybrid state space, a result that is inspired by the Joint Spectral Radius theorem. This leads to an algorithm for computing the maximum stable delay exactly. Other potential applications of our technique include co-simulation, networked control systems and delayed controlled switching with a state feedback control.

==> Makefile <==
# You can change the pdf viewer to your preferred
# one by commenting every line beginning by
# `PDFVIEWER' except the one with your pdf viewer
PDFVIEWER=evince # GNOME
#PDFVIEWER=okular # KDE
#PDFVIEWER=xpdf # lightweight
#PDFVIEWER=xdg-open # Default pdf viewer - GNU/Linux
#PDFVIEWER=open # Default pdf viewer - Mac OS
MAIN_NAME=root
PDF_NAME=$(MAIN_NAME).pdf

# You want latexmk to *always* run, because make does not have all the info.
.PHONY: $(PDF_NAME) clean show release

# If you want the pdf to be opened by your preferred pdf viewer
# after `$ make', comment the following line and uncomment the
# line after
#default: all
default: show

all: $(PDF_NAME)

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interactive=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

# Other depences are gessed automatically by latexmk
# see http://tex.stackexchange.com/questions/40738/how-to-properly-make-a-latex-project
$(PDF_NAME): $(MAIN_NAME).tex
	latexmk -pdf -pdflatex="pdflatex -shell-escape -enable-write18" \
	  -use-make $(MAIN_NAME).tex

clean:
	latexmk -CA

show: $(PDF_NAME)
	$(PDFVIEWER) $(PDF_NAME) 2> /dev/null &

release: all
	smartcp -v config.yml


==> bouncingball_equations.tex <==
\section{Bouncing ball example equations}
\label{sec:bb_equations}

The free fall mode is dictated by the following ordinary differential equation:
\begin{equation}\label{eq:mode2}
\dert{x} = f_2(x) = \vectorTwo{x_2}{- \frac{d_a}{m} x_2 \abs{x_2} - g},
\end{equation}
\noindent where $x_i$ denotes the $i$-th component of vector $x$, with $x_1$ the position and $x_2$ the velocity, and $m,d_a,g$ denote the mass, air drag, and gravity constants, respectively.

The contact mode captures the dynamics of the ball for the brief moments it is in contact with the floor, governed by the following system:
\begin{equation}\label{eq:mode1}
\dert{x} = f_1(x) = \vectorTwo{x_2}{\frac{c}{m}(r - x_1) - \frac{d_c}{m} x_2 - \frac{d_a}{m} x_2 \abs{x_2} - g},
\end{equation}
\noindent where $d_c,c,r$ denote the compression damping, stiffness, and the ball radius, respectively.

The parameters used throughout this document were taken from \cite{Fontanella2008}:
$r = \SI{0.25}{\meter}$,
$m = \SI{0.650}{\kilogram}$,
$c = \SI{40000}{\newton\per\meter}$,
$d_c = \SI{10}{\newton\per\meter}$,
$d_a = \SI{0.0136}{\newton\per\meter\squared}$, and
$g = \SI{9.81}{\meter\per\second\squared}$.


==> reachability_analysis.tex <==
\section{Reachability Analysis with SpaceEx}
\label{sec:reachability}

Reachability techniques can be used to approximate $\sigma(\SD)$ by trial an error.
For example, replacing the non-linear drag term in the bouncing ball example ($- d_a/m x_2 \abs{x_2}$ in \ceqreff{eq:mode2}{eq:mode1}) by a linear term $-d_a/m$ with $d_a=10^{-6}$, allows us to use SpaceEx~\cite{Frehse2011} with the model depicted in \cref{fig:spaceex_model}.
Applying our algorithm to the affine bouncing ball model with $h_1=0$, yields the values for $h_2$ as plotted in \cref{fig:h2_plot_affine}.
The minimum is ${\opt{h_2}(x, 0.0)}=0.001623205$ at $x=-0.4991045$.
To check these results, we ran SpaceEx with the initial conditions $x=-0.4991045,v=0.0$ and parameters $h_1=0,0<h_2<0.001623205$.
A fixed point was not reached, but the intermediate state space, shown in \cref{fig:spaceex_output}, hints at the correctness of our result: the trajectories do not reach $x<-0.4991045$.
Compared to our algorithm, this trial and error process to find the solution to \ceqref{eq:2Dopt} is not feasible in practice, but can be used to check the solution found.

\begin{figure}
  \centering
  \begin{tikzpicture}[scale=0.99]
  \begin{axis}[
  width=\defaultImageWidth\textwidth,
  yscale=0.5,
  xlabel=$x$,
  ylabel=${\opt{h_2}(x, 0.0)}$]
  \addplot[color=agro, thick,mark=o] coordinates {
    (-0.763932022500210,0.001623222980134)
    (-0.700000000000000,0.001623216189219)
    (-0.618033988749895,0.001623209520900)
    (-0.600000000000000,0.001623208424548)
    (-0.511105363561801,0.001623205407812)
    (-0.508327499050959,0.001623205389871)
    (-0.501285614686153,0.001623205364357)
    (-0.500000000000000,0.001623205363082)
    (-0.499238544308164,0.001623205362839)
    (-0.499148683174635,0.001623205362950)
    (-0.499114359275894,0.001623205362831)
    (-0.499101248713202,0.001623205362814)
    (-0.499093145939846,0.001623205362822)
    (-0.499073160443430,0.001623205362832)
    (-0.498962867447096,0.001623205362830)
    (-0.489891606439050,0.001623205391418)
    (-0.460061705580038,0.001623205910075)
    (-0.381966011250105,0.001623210865408)
  };
  \end{axis}
  \end{tikzpicture}
  \caption{Affine bouncing ball model results. Plot of $\opt{h_2}(x, h_1)$ as a function of the point of
    the \PCRay{}, and $h_1=0$ (recall \ceqref{eq:2Dopt}).}
  \label{fig:h2_plot_affine}
\end{figure}

\begin{figure}[htb]
  \begin{center}
    \begin{subfigure}[b]{0.4\textwidth}
      \includegraphics[width=\textwidth]{spaceex_model}
      \caption{Delayed transition SpaceEx affine model of the bouncing ball example.}
      \label{fig:spaceex_model}
    \end{subfigure}
    ~ %
    \begin{subfigure}[b]{0.3\textwidth}
      \includegraphics[width=\textwidth]{spaceex_output}
      \caption{Clipped state space output, produced with SpaceEx. The horizontal axis refers to position, and vertical refers to velocity.}
      \label{fig:spaceex_output}
    \end{subfigure}
  \end{center}
  \caption{SpaceEx results.}
\end{figure}

